Feature Unlearning for Pre-trained GANs and VAEs

We tackle the problem of feature unlearning from a pre-trained image generative model: GANs and VAEs. Unlike a common unlearning task where an unlearning target is a subset of the training set, we aim to unlearn a specific feature, such as hairstyle from facial images, from the pre-trained generative models. As the target feature is only presented in a local region of an image, unlearning the entire image from the pre-trained model may result in losing other details in the remaining region of the image. To specify which features to unlearn, we collect randomly generated images that contain the target features. We then identify a latent representation corresponding to the target feature and then use the representation to fine-tune the pre-trained model. Through experiments on MNIST, CelebA, and FFHQ datasets, we show that target features are successfully removed while keeping the fidelity of the original models. Further experiments with an adversarial attack show that the unlearned model is more robust under the presence of malicious parties.

==> algorithms/unlearning_framework.tex <==
\begin{algorithm}[t]
    \caption{Feature Unlearning}
    \label{alg:unlearning}
    \begin{algorithmic}
        \REQUIRE Pre-trained generator $f$
%        \REQUIRE pre-trained generator $f$
        \REQUIRE $E$: number of epochs, $\alpha$: hyper-parameter
%        \STATE {\bfseries Output:} 
        
        \STATE Collect the positive and negative examples
        \STATE Compute mean vector $\rvz_p$ from the positive samples
        \STATE Compute mean vector $\rvz_n$ from the negative samples
        % \STATE Compute latent vector $Z_e = \{f^{-1}(x) \mid x \in D_e\}$
        % \STATE Get latent vector $\rvz_{{\mathcal{D}}_e}$ of $\mathcal{D}_e$
        \STATE Compute target vector $\rvz_e = \rvz_p - \rvz_n$
        \STATE Initialize $g_{\theta} = f$
        \FOR{$i=1$ {\bfseries to} $E$}
            \STATE Sample $\rvz$ from $N(0,1)$ and compute $\operatorname{sim}(\rvz, \rvz_e)$
            \STATE Compute $\nabla_\theta \mathcal{L}(\theta)$ %(\alpha \cdot \mathcal{L}_{\textrm{unlearn}}(\theta) + \mathcal{L}_{\textrm{recon}}(\theta))$ 
            \STATE Update $\theta\leftarrow\theta - \nabla_\theta\mathcal{L}(\theta)$ %(\alpha \cdot \mathcal{L}_{\textrm{unlearn}}(\theta) + \mathcal{L}_{\textrm{recon}}(\theta))$
        \ENDFOR

        \RETURN Unlearned generator $g_\theta$
    \end{algorithmic}
\end{algorithm}

% , All experiments in this paper used the default values $E=100$, $m=1,000$, $\alpha=0.02$

==> tables/diversity.tex <==
% \begin{table}[h!]
% \label{table/diversity}
% \begin{tabular}{ccccc}
% \centering
% \vskip 0.05in
% \begin{small}
% \toprule
%      & \multicolumn{2}{c}{Bang} & \multicolumn{2}{c}{Beard} \\ 
%      & Unlearn    & Baseline    & Unlearn     & Baseline    \\
% Top5 & 0.008      & 0.028       & 0.040       & 0.036       \\
% All  & 0.012      & 0.099       & 0.120       & 0.107       \\ \bottomrule
% \end{small}
% \end{tabular}
% \end{table}

\begin{table}[t!]
\centering
\caption{Quantitative analysis of diversity. We evaluate the feature diversity by calculating the difference in feature ratio between the original model. The `Top3' represents the average feature ratio difference for the three most correlated features to the target feature, while `all' represents the average feature ratio difference for all features.}
\label{table/diversity}
\vskip 0.05in
\begin{small}
\begin{tabular}{crrrr}
\toprule
& \multicolumn{2}{c}{Bang} & \multicolumn{2}{c}{Beard} \\ \midrule
 & Unlearn    & Baseline    & Unlearn     & Baseline    \\ \midrule
Top3 & 0.008      & 0.028       & 0.040       & 0.036       \\
All  & 0.012      & 0.099       & 0.120       & 0.107       \\ \bottomrule
\end{tabular}

\end{small}
\end{table}

% 0.028711509 for bang
% 0.008797733
% 0.09914428
% 0.01281476


% 0.03616901 for beard
% 0.040665247
% 0.10735127
% 0.120452054

==> tables/symbols.tex <==
\begin{table}[t]
\caption{Summary of symbols}
\label{table/symbols}
\centering
\vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{tabular}{c|c}
    \toprule
    Symbol & Meaning \\
    \midrule
    $\mathfrak{A}$ & Unlearning algorithm\\  
    $f$ & Pre-trained generative model \\
    $g_{\theta}$ & Target generator to unlearn \\
    $\mathcal{D}$ & Dataset\\
    $\mathcal{D}_e$ & Target data to be erased \\
    $\rvz,\mathcal{Z}$ & Latent vector, latent space\\
    $\rvz_e$ & Target attribute vector\\
    % $\mathcal{I}_t$ & Images that has the target attribute $t$\\
    % % \textit{non-target image}& Image that doesn't has a target attribute\\
    \bottomrule
    \end{tabular}
    \end{small}
    \end{center}
\vskip -0.1in
\end{table}

